Choreographies as Macros

Concurrent programming often entails meticulous pairing of sends and receives between participants to avoid deadlock. Choreographic programming alleviates this burden by specifying the system as a single program. However, there are more applications than implementations of choreographies, and developing new implementations takes a lot of time and effort. Our work uses Racket to expedite building a new choreographic language called Choret. Racket has a powerful macro system which allows Choret to reuse much of its infrastructure for greater functionality and correctness.

==> eptcsdata.tex <==
\providecommand{\firstpage}{12}
\providecommand{\publicationstatus}{Farzaneh Derakhshan \& Jan Hoffmann (Eds.): 16th International\\ Workshop on
Programming Language Approaches to Concurrency\\
and Communication-cEntric Software 2025 (PLACES 2025)\\
EPTCS 420, 2025, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.420.2}{10.4204/EPTCS.420.2}}
\pdfoutput=1

